Minimum-Risk Recalibration of Classifiers

Recalibrating probabilistic classifiers is vital for enhancing the reliability and accuracy of predictive models. Despite the development of numerous recalibration algorithms, there is still a lack of a comprehensive theory that integrates calibration and sharpness (which is essential for maintaining predictive power). In this paper, we introduce the concept of minimum-risk recalibration within the framework of mean-squared-error (MSE) decomposition, offering a principled approach for evaluating and recalibrating probabilistic classifiers. Using this framework, we analyze the uniform-mass binning (UMB) recalibration method and establish a finite-sample risk upper bound of order $\tilde{O}(B/n + 1/B^2)$ where $B$ is the number of bins and $n$ is the sample size. By balancing calibration and sharpness, we further determine that the optimal number of bins for UMB scales with $n^{1/3}$, resulting in a risk bound of approximately $O(n^{-2/3})$. Additionally, we tackle the challenge of label shift by proposing a two-stage approach that adjusts the recalibration function using limited labeled data from the target domain. Our results show that transferring a calibrated classifier requires significantly fewer target samples compared to recalibrating from scratch. We validate our theoretical findings through numerical simulations, which confirm the tightness of the proposed bounds, the optimal number of bins, and the effectiveness of label shift adaptation.

==> archive/02_preliminaries.tex <==
\section{Preliminaries}\label{sec:preliminaries}

\subsection{Notation}
Let $\NN$ and $\RR$ denote the set of positive integers and the set of real numbers, respectively. 
For $n\in\mathbb{N}$, let $[n]:=\{1,\dots,n\}$. 
For $x\in\mathbb{R}$, let $\lfloor x \rfloor = \max\{m\in \mathbb {Z}: m\leq x\}$.
For any finite set $\cS = \{ s_i: i \in [n] \} \subset \RR$ and any $k \in [n]$, we let $s_{(k)}$ denote the $k$-th order statistics, which is the $k$-th smallest element in $\cS$.
% ; therefore, $s_{(1)} \leq s_{(2)} \leq \dots \leq s_{(n)}$.

Let $(\Omega, \cE, P)$ denote a generic probability space. %, where $\Omega$ is the sample space, $\cE$ is a $\sigma$-algebra on $\Omega$, and $P$ is a probability measure. 
For an event $A \in \cE$, the indicator function $\indic_A: \Omega \to \{0,1\}$ is defined such that $\indic_A(x) = 1$ if and only if $x \in A$. 
We write $A$ happens $P$-almost surely if $P(A) = 1$. 
%
For a random variable $X: \Omega \to \RR^d$, we let $\sigma(X) := \left\{ X^{-1}(A): A \in \borel(\RR^d) \right\}$ denote the $\sigma$-algebra generated by $X$, where $\borel(\RR^d)$ is the Borel $\sigma$-algebra on $\RR^d$. 
%Furthermore, we denote by $L^1(\Omega, \mathcal{E}, P)$ and $L^2(\Omega, \mathcal{E}, P)$ the sets of integrable and square-integrable random variables, respectively. 
For $x \in \RR^d$, let $\delta_x$ denote the Dirac measure on $\RR^d$, defined as $\delta_x(A) = \indic_A(x)$ for all $A \in \cB(\RR^d)$. 
% We may identify a finite set $\cD$ with its empirical measure $\emp_{\cD} = \frac{1}{|\cD|}\sum_{x \in \cD} \delta_x$. 
For a probability measure $P$, define $\EP$ as the expectation, with subscript $P$ omitted when the underlying probability measure is clear.
For a probability measure $P$ and a random variable $X: \Omega \to \RR^d$,
let $P_X:=P\circ X^{-1}$ be the probability measure induced by $X$,  % $P_X: \borel(\RR^d) \to [0, 1]$
and let $P[X\in B]:= P(\{\omega: X(\omega) \in B\})$ for any $B\in \borel(\RR^d)$.
%%%% Rigorous definitions in probability theory
% For a probability measure $P$ and a random variable $X,Y$,
% let $P_X:=P\circ X^{-1}$ be the probability measure induced by $X$;
% let $P[X\in B]:= P(\{\omega: X(\omega) \in B\})$ for Borel set $B$;
% let $\EP[Y | \mathcal{A}]$ be the conditional expectation of $Y$ given sub-$\sigma$-algebra $\cA \subseteq \cE$, which is the unique $\cA$-measurable random variable such that $E[\indic_A \EP[Y \mid \cA]] = E[\indic_A Y]$ for any $A \in \cA$;
% let $\EP[Y \mid X] := \EP[Y \mid \sigma(X)]$ and $P(A \mid X) := E[\indic_A \mid \sigma(X)]$ for any $A\in\cE$.

%we overload $P$ to denote the joint/marginal/conditional measures that are induced by random variable(s), but its meaning should be clear from the context (otherwise, we add subscript). 
% With an underlying probability measure specified, we use $\bbP$ and $\bbE$ denote the probability and the expectation.

Letting $f, g:\RR \to \RR$, we write $f(x) = O(g(x))$ as $x\to\infty$ if there exist $M>0$ and $x_0 > 0$ such that $\left| f(x) \right| \leq M g(x)$ for all $x\geq x_0$. 
Likewise, we write $f(x) = \Omega(g(x))$ if $g(x) = O(f(x))$. 
Furthermore, we write $f(x) = o(g(x))$ as $x\to\infty$ if $\lim_{x\to\infty} \frac{f(x)}{g(x)} = 0$.



\subsection{Probability Calibration for Prediction}
Consider the binary classification problem; let $\cX \subset \RR^d$ and $\cY = \{0,1\}$ denote the feature and label spaces. 
Letting $P$ denote a joint distribution of random variable $(X,Y): \Omega \to \cX \times \cY$, we want to construct a function $f: \cX \to \cZ = [0,1]$ that estimates the conditional probability, \ie,
\begin{equation}\label{eqn:ideal}
    f(X) \approx \bbP( Y=1 \mid X ).
\end{equation}
However, this approximate equality may not hold, even for classifiers that can accurately predict $y$ given $x$.


\paragraph{Calibration.} 
The notion of calibration captures the intuition in the approximate equality \eqref{eqn:ideal}, but in a weaker sense. 
Here we introduce the widely-adopted notion of perfect calibration \cite{murphy1967verification,dawid1982well,gupta2020predictionset}.
\begin{definition}\label{def:calibration}
    A function $f: \cX \to \cZ$ is \emph{(perfectly) calibrated} with respect to distribution $P$, if
    \[
        f(X) = \bbP \left[Y=1 \mid f(X) \right]     \quad \textrm{ $P$-almost surely.}
    \]
\end{definition}
For a given classification problem, there are typically many calibrated models. 
Vaicenavicius \etal \cite{vaicenavicius2019evaluating} characterized the functions $f$ that achieve perfect calibration; see \cite[Proposition 1]{gupta2020predictionset}, too.
\begin{proposition}[{\cite[Proposition 1]{vaicenavicius2019evaluating}}]\label{prop:char_calib}
    A function $f: \cX \to \cZ$ is perfectly calibrated if and only if there exists a measurable space $\cZ'$ and a measurable function $g: \cX \to \cZ'$ such that
    \begin{equation}
        f(X) = \bbP \left[ Y=1 \mid g(X) \right]    \quad \textrm{ $P$-almost surely.}
    \end{equation}
\end{proposition}


Here we briefly review other notions of calibration used in the literature. 
A random predictor $f(X)$ is said to be auto-calibrated when $f$ is perfectly calibrated \cite{tsyplakov2013evaluation, gneiting2013combining}.
In multi-class classification, weaker notions of calibration exist, including confidence calibration \cite{gupta2021top}, top-label calibration\footnote{Unfortunately, top-label calibration is sometimes referred to as perfect calibration in machine learning community, \eg, \cite{guo2017calibration}, which can be confusing as pointed out by Vaicenavicius \etal \cite{vaicenavicius2019evaluating}.} \cite{kumar2019verified,gupta2021top}, and class-wise calibration \cite{zadrozny2002transforming,kull2019beyond,gupta2020splines}, to name a few. 
These weaker notions of calibration only conditions on narrower aspects of the prediction, such as the highest predicted probabilities among multiple classes in top-label calibration. 
% \footnote{\zs{$\mathbb{P}(\hat{Y}=Y \mid \hat{P}=p)=p, \quad \forall p \in[0,1]$}}
For binary classification, these notions of calibration are all equivalent to perfect calibration.
Finally, it is worth noting that the concept of calibration is not limited to classification, but is also widely studied in the context of regression \cite{kuleshov2018accurate,song2019distribution} and with respect to general statistical functionals \cite{gneiting2021regression,gneiting2023model}.


\paragraph{Recalibration Methods.} 
Many machine learning algorithms do not automatically produce well-calibrated probabilistic predictors out of the box, which raise concerns about their reliability, especially for safety-critical applications. 
To address this issue, one can find a post-processing function that corrects the predicted probabilities and makes the predictors calibrated. 
Formally, for an arbitrary predictor $f: \cX \to \cZ$, the aim of recalibration is to identify a post-processing function $h:\cZ\to\cZ$ such that $h\circ f$ is perfectly calibrated. 
This problem can be viewed as a regression problem, where we estimate the function $h(z) \approx \bbE[Y \mid Z=z]$ given a calibration dataset $\left\{ (x_i, y_i, z_i): i \in [n] \right\}$, where $z_i=f(x_i)$, $\forall i \in [n]$; see Section \ref{sec:setup} for more details.


\paragraph{Beyond Calibration: Sharpness.}
While calibration is an important prerequisite for reliable prediction, calibration itself is not sufficient to produce a useful predictor. 
For instance, a constant predictor $f(X) = \bbE Y$ (which is obtained by setting $g(X) = c$ for any constant $c$ in Proposition \ref{prop:char_calib}) is perfectly calibrated, but it is not informative as it does not utilize feature information at all. 
Thus, additional properties are desired for accurate and reliable probabilistic forecast. 
One of such properties is the so-called sharpness \cite{murphy1973new}, also known as resolution or refinement \cite{jolliffe2012forecast}, which is also related to the notion of sufficiency \cite{tasche2021calibrating}. 
\begin{definition}\label{def:sharpness}
    The \emph{sharpness} of a function $f: \cX \to \cZ$ with respect to distribution $P$ refers to the quantity
    \[
        \var\big( \bbE[Y\mid f(X)] \big) = \bbE \Big[ \big( \bbE[Y\mid f(X)] - \bbE[Y] \big)^2 \Big].
    \]
\end{definition}
Intuitively speaking, sharpness measures the variation in the true probability across forecasts. 
The following decomposition of the mean squared error (MSE) suggests why it is desirable for a classifier $f$ to be calibrated and have high sharpness; note that $\var[ Y ]$ is a quantity intrinsic to the problem, unrelated to $f$.
\begin{equation}
    \MSE(f) := \underbrace{\bbE\big[ \big( Y - f(X) \big)^2 \big]}_{\textrm{mean-squared error}}
        = \var[ Y ] - \underbrace{\var\left( \bbE \big[Y\mid f(X)\big] \right)}_{\textrm{sharpness}} + \underbrace{\bbE \big[ \big( f(X) - \bbE[Y\mid f(X)] \big)^2 \big]}_{\textrm{lack of calibration}}
\end{equation}

% \DS{It may helpful to add examples of
% (1) sharp, but highly uncalibrated predictor, and (2) a calibrated, but not sharp predictor.}

==> archive/02_theory_new.tex <==
\section{Optimal recalibration}
\label{sec:theory_opt}
% Motivation:
% In the current paper, we define the \REL and \GRP risks, and use them to define the recalibration risk, then we identify the optimal recalibration $h^*$.
% However, it is more principled to define the calibration and sufficiency, which don't requires definition of any loss/risks. Then we claim there is one and only one $h^*$. The we use $L_2$ distance to measure the risks.

\subsection{Notation}
Let $\NN$ and $\RR$ denote the set of positive integers and the set of real numbers, respectively. 
For $n\in\mathbb{N}$, let $[n]:=\{1,\dots,n\}$. 
For $x\in\mathbb{R}$, let $\lfloor x \rfloor = \max\{m\in \mathbb {Z}: m\leq x\}$.
For any finite set $\cS = \{ s_i: i \in [n] \} \subset \RR$ and any $k \in [n]$, we let $s_{(k)}$ denote the $k$-th order statistics, which is the $k$-th smallest element in $\cS$.
% ; therefore, $s_{(1)} \leq s_{(2)} \leq \dots \leq s_{(n)}$.

Let $(\Omega, \cE, P)$ denote a generic probability space. %, where $\Omega$ is the sample space, $\cE$ is a $\sigma$-algebra on $\Omega$, and $P$ is a probability measure. 
For an event $A \in \cE$, the indicator function $\indic_A: \Omega \to \{0,1\}$ is defined such that $\indic_A(x) = 1$ if and only if $x \in A$. 
We write $A$ happens $P$-almost surely if $P(A) = 1$. 
%
For a random variable $X: \Omega \to \RR^d$, we let $\sigma(X) := \left\{ X^{-1}(A): A \in \borel(\RR^d) \right\}$ denote the $\sigma$-algebra generated by $X$, where $\borel(\RR^d)$ is the Borel $\sigma$-algebra on $\RR^d$. 
%Furthermore, we denote by $L^1(\Omega, \mathcal{E}, P)$ and $L^2(\Omega, \mathcal{E}, P)$ the sets of integrable and square-integrable random variables, respectively. 
For $x \in \RR^d$, let $\delta_x$ denote the Dirac measure on $\RR^d$, defined as $\delta_x(A) = \indic_A(x)$ for all $A \in \cB(\RR^d)$. 
% We may identify a finite set $\cD$ with its empirical measure $\emp_{\cD} = \frac{1}{|\cD|}\sum_{x \in \cD} \delta_x$. 
For a probability measure $P$, define $\EP$ as the expectation, with subscript $P$ omitted when the underlying probability measure is clear.
For a probability measure $P$ and a random variable $X: \Omega \to \RR^d$,
let $P_X:=P\circ X^{-1}$ be the probability measure induced by $X$,  % $P_X: \borel(\RR^d) \to [0, 1]$
and let $P[X\in B]:= P(\{\omega: X(\omega) \in B\})$ for any $B\in \borel(\RR^d)$.
%%%% Rigorous definitions in probability theory
% For a probability measure $P$ and a random variable $X,Y$,
% let $P_X:=P\circ X^{-1}$ be the probability measure induced by $X$;
% let $P[X\in B]:= P(\{\omega: X(\omega) \in B\})$ for Borel set $B$;
% let $\EP[Y | \mathcal{A}]$ be the conditional expectation of $Y$ given sub-$\sigma$-algebra $\cA \subseteq \cE$, which is the unique $\cA$-measurable random variable such that $E[\indic_A \EP[Y \mid \cA]] = E[\indic_A Y]$ for any $A \in \cA$;
% let $\EP[Y \mid X] := \EP[Y \mid \sigma(X)]$ and $P(A \mid X) := E[\indic_A \mid \sigma(X)]$ for any $A\in\cE$.

%we overload $P$ to denote the joint/marginal/conditional measures that are induced by random variable(s), but its meaning should be clear from the context (otherwise, we add subscript). 
% With an underlying probability measure specified, we use $\bbP$ and $\bbE$ denote the probability and the expectation.

Letting $f, g:\RR \to \RR$, we write $f(x) = O(g(x))$ as $x\to\infty$ if there exist $M>0$ and $x_0 > 0$ such that $\left| f(x) \right| \leq M g(x)$ for all $x\geq x_0$. 
Likewise, we write $f(x) = \Omega(g(x))$ if $g(x) = O(f(x))$. 
Furthermore, we write $f(x) = o(g(x))$ as $x\to\infty$ if $\lim_{x\to\infty} \frac{f(x)}{g(x)} = 0$.


\subsection{Preliminaries}
Consider the binary classification problem; let $\cX \subset \RR^d$ and $\cY = \{0,1\}$ denote the feature and label spaces. 
Letting $P$ denote a probability measure and $(X,Y): \Omega \to \cX \times \cY$ denote a pair of jointly distributed random variables, we want to construct a function $f: \cX \to \cZ = [0,1]$ that estimates the conditional probability, \ie,
\begin{equation}\label{eqn:ideal}
    f(X) \approx \bbP[ Y=1 \mid X ] = \bbE_P [ Y \mid X].
\end{equation}

We first introduce two notions regarding probabilistic classifiers that exists in the literature: calibration \cite{murphy1967verification,dawid1982well,gupta2020predictionset} and sufficiency \cite{tasche2021calibrating}.
\begin{definition}\label{def:calibration}
    A function $f: \cX \to \cZ$ is \emph{(perfectly) calibrated} with respect to distribution $P$, if
    \[
        f(X) = \bbP \left[Y=1 \mid f(X) \right]     \quad \textrm{ $P$-almost surely.}
    \]
\end{definition}
Calibrated classifiers are in general not unique: given an arbitrary measurable space $\cZ'$ and a measurable function $g: \cX \to \cZ$, the function $f:\cX \to \cZ$ such that $f(X) = \bbE [Y \mid g(X)]$, $P$-almost surely is calibrated.
In fact, this can be extended to a characterization of calibrated functions, as the converse is also true \cite[][Proposition 1]{gupta2020predictionset}. % converse: (every calibrated classifier assumes the above form of conditional expectation)

Given any classifier $f$, 
Note that calibration itself does not guarantee a useful predictor.
For instance, a constant predictor $f(X) = \bbE Y$ is perfectly calibrated, but it ignores the information in features.
% The notion of sufficiency says we don't loose any information in terms of predicting $Y$ conditioned on a coarser $\sigma$-algebra \cite{tasche2021calibrating}.
The notion of sufficiency says we don't lose any resolution in terms of predicting $Y$ conditioned on a processed classifier \cite{tasche2021calibrating}.
\begin{definition}\label{def:sufficiency}
    A function $g: \cX \to \cZ$ is \emph{sufficient} for another function $f: \cX \to \cZ$ with respect to $Y$ under probability measure $P$ if
    \[
        \bbE_P \left[ Y \mid h(f(X)) \right] = \bbE_P \left[ Y \mid f(X) \right] \quad \textrm{ $P$-almost surely.}
    \]
\end{definition}
Note that the notion of sufficiency is not dependent on the notion of calibration. For example, any injective $h$ yields $h \circ f$ that is sufficient for $f$.

% \paragraph{Sharpness}
% Calibration itself is not sufficient to produce a useful predictor.
% For instance, a constant predictor $f(X) = \bbE Y$ is perfectly calibrated, but it is not informative as it does not utilize feature information at all. 
% Another desired property for probabilistic forecast is sharpness \cite{murphy1973new}, also known as resolution \cite{jolliffe2012forecast}. %, which is also related to the notion of sufficiency \cite{tasche2021calibrating}. 
% \begin{definition}\label{def:sharpness}
%     The \emph{sharpness} of a function $f: \cX \to \cZ$ with respect to distribution $P$ refers to the quantity
%     \[
%         \var\big( \bbE[Y\mid f(X)] \big) = \bbE \Big[ \big( \bbE[Y\mid f(X)] - \bbE[Y] \big)^2 \Big].
%     \]
% \end{definition}
% Intuitively, sharpness measures the explained variance in the target $Y$ by the prediction $f(X)$. 
% The following decomposition of the mean squared error (MSE) suggests why it is desirable for a classifier $f$ to be calibrated and have high sharpness; note that $\var[ Y ]$ is a quantity intrinsic to the problem, unrelated to $f$.
% \begin{equation}
%     \MSE(f) := \underbrace{\bbE\big[ \big( Y - f(X) \big)^2 \big]}_{\textrm{mean-squared error}}
%         = \var[ Y ] - \underbrace{\var\left( \bbE \big[Y\mid f(X)\big] \right)}_{\textrm{sharpness}} + \underbrace{\bbE \big[ \big( f(X) - \bbE[Y\mid f(X)] \big)^2 \big]}_{\textrm{lack of calibration}}
% \end{equation}

% \paragraph{Sufficiency} Inspired by the concept of sufficient $\sigma$-algebra in \cite{tasche2021calibrating}, we introduce the notation of sufficient prediction functions.

% \zs{Injective functions}

\subsection{Optimal Recalibration}
% sufficient calibrator
Many machine learning algorithms do not automatically produce calibrated classifiers.
To address this issue, one can find a post-processing function that corrects the predicted probabilities and makes the classifiers calibrated.
In addition, it is also desired the calibrated classifier is sufficient for the original classifier so that no information regarding $Y$ is lost.
The following theorem states that there exists an essentially unique calibration function that meet both requirements.
\begin{theorem}\label{Thm:opt}
    Given probability measure $P$, random variables $(X, Y): \Omega \to \cX \times \cY$, and function $f:\cX \to \cZ$, there exists a function $h^*: \cZ \to \cZ$ such that $h \circ f$ is perfectly calibrated and sufficient for $f$ with respect to $Y$.
    Moreover, $h^*$ is unique up to a $P$-null set on the support of $f(X)$:
    $$h^*(z) = \bbE_P [Y \mid f(X)=z], \qquad z\in\supp{P_{f(X)}}.$$
\end{theorem}

We call the unique sufficient calibration function as According to Theorem~\ref{Thm:opt}, without loss of generality, we construct $h^*$ as
\begin{align}
    h^*_{f,P}(z) = \begin{cases}
        \bbE_P [Y \mid f(X)=z], & z\in\supp{P_{f(X)}} \\
        0, & z\notin\supp{P_{f(X)}}.
    \end{cases}
\end{align}
Then we can define the \emph{recalibration risk} of any recalibration function $h: \cZ \to \cZ$ using the squared error loss:
Theorem~\ref{Thm:opt} motivates us to define the \emph{recalibration risk} of $h$ as follows:
\begin{equation}\label{eqn:risk_recalib}
    R(h) = R_P(h; f, P) := \bbE_P \left[(h\circ f(X) - \bbE_P[Y \mid f(X)])^2 \right].
\end{equation}

These requirements can be quantified using the following two notions of risks.

\begin{definition}\label{defn:calibration_risk}
    Let $f: \cX \to \cZ$. The \emph{calibration risk} of $f$ under $P$ is defined as
    \begin{equation}\label{eqn:loss_rel}
        \REL(h) = \REL(h; f, P) := \bbE \left[ \big( f(X) - \bbE\left[ Y \mid f(X) \right] \big)^2 \right].
    \end{equation}
\end{definition}

\begin{definition}\label{defn:sharpness_risk}
   Let $f: \cX \to \cZ$ and $h: \cZ \to \cZ$. The \emph{sharpness risk} of $h$ over $f$ under $P$ is defined as 
    \begin{equation}\label{eqn:loss_grp}
        \GRP(h) = \GRP(h; f, P) := \bbE \left[ \big( \bbE\left[ Y \mid h \circ f(X) \right] - \bbE\left[ Y \mid f(X) \right] \big)^2 \right].
    \end{equation}
\end{definition}

We can see $\REL(h) = 0$ if and only if $h \circ f$ is perfectly calibrated, cf. Definition~\ref{def:calibration}; $\REL(h) = 0$ if and only if $h \circ f$ is sufficient for $f$, cf. Definition~\ref{def:sufficiency}.




% Formally, given a probabilistic classifier $f: \cX \to \cZ$, the aim of recalibration is to identify a post-processing function $h:\cZ\to\cZ$ such that $h\circ f$ is perfectly calibrated. 
% This problem can be viewed as a regression problem, where we estimate the function $h(z) \approx \bbE[Y \mid Z=z]$ given a calibration dataset $\left\{ (x_i, y_i, z_i): i \in [n] \right\}$, where $z_i=f(x_i)$, $\forall i \in [n]$; see Section \ref{sec:setup} for more details.





==> archive/03_optimal_recalibration.tex <==
\section{Optimal Recalibration}  \label{sec:opt_cal}
% This section is organized as follows. 
% In Section~\ref{sec:setup}, we formulate the problem of recalibration and define the risk function that can be used to evaluate a recalibration scheme. 
% In Section~\ref{sec:est_hp}, we describe an algorithm for recalibration, which is based on the so-called uniform-mass binning method. 
% In Section \ref{sec:analysis}, we provide theoretical analysis on the performance of the proposed method. 
% Specifically, 

\subsection{Revisiting the Decomposition of Mean-squared Error}    \label{sec:decomp}

Let us recall that $\cX \subset \RR^d$, $\cY = \{0,1\}$, and $\cZ = [0,1]$. 
Suppose that we have a function $f: \cX \to \cZ$ and $P$ is a joint distribution of a random variable $(X,Y) \in \cX \times \cY$. 
As we want to estimate a recalibration function $h: \cZ \to \cZ$, we need a measure to evaluate $h$. 
Here we introduce two notions of risk.

\begin{definition}\label{defn:calibration_risk}
    Let $f: \cX \to \cZ$. The \emph{calibration risk} of $f$ under $P$ is defined as
    \begin{equation}\label{eqn:loss_rel}
        \REL(f) = \REL(f; P) := \bbE \left[ \big( f(X) - \bbE\left[ Y \mid f(X) \right] \big)^2 \right].
    \end{equation}
\end{definition}
\begin{definition}\label{defn:sharpness_risk}
   Let $f: \cX \to \cZ$ and $h: \cZ \to \cZ$. The \emph{sharpness risk} of $h$ over $f$ under $P$ is defined as 
    \begin{equation}\label{eqn:loss_grp}
        \GRP(h) = \GRP(h; f, P) := \bbE \left[ \big( \bbE\left[ Y \mid h \circ f(X) \right] - \bbE\left[ Y \mid f(X) \right] \big)^2 \right].
    \end{equation}
\end{definition}

Firstly, observe that the calibration risk $\REL$ measures how well-calibrated $f$ is, cf. Definition \ref{def:calibration}. 
Secondly, the sharpness risk quantifies the decrement in sharpness of $f$ incurred by applying the recalibration map $h$. 
%
It is known that $\GRP(h; f)=0$ if and only if $h\circ f(X)$ is sufficient for $f (X)$ with respect to $Y$, which can be achieved when $\sigma\big( h \circ f (X) \big) = \sigma \big( f(X) \big)$ \cite{tasche2021calibrating}. 


Indeed, the MSE of $h \circ f$ can be decomposed into these two types of risks, plus an additional term that is independent of $h$. 
We state this result in the following proposition, whose proof is deferred to Appendix~\ref{sec:risk_decomp_additional}.

\begin{proposition}[Calibration-sharpness decomposition]\label{Prop:risk_decomposition}
    For any $f: \cX \to \cZ$ and any $h: \cZ \to \cZ$,
    \begin{equation}
    \begin{split}
        %\bbE\left[ \big( Y - h \circ f(X) \big)^2 \right] 
        \MSE( h \circ f )
            &= \bbE\left[ \big( h\circ f(X) - \bbE[ Y \mid f(X) ] \big)^2 \right]
                +  \bbE\left[ \big( Y - \bbE[Y\mid f(X)] \big)^2 \right]\\
            &= \REL\left( h\circ f; P \right) + \GRP \left( h; f, P \right)
                + \bbE\left[ \big( Y - \bbE[Y\mid f(X)] \big)^2 \right].
    \end{split}
    \end{equation}
\end{proposition}

Proposition \ref{Prop:risk_decomposition} states that the MSE of the recalibrated classifier $h \circ f$ can be decomposed to three terms: (1) the calibration risk of $h \circ f$; (2) the sharpness risk of $h$ over $f$; and (3) the residual term that does not depend on the $h$.
Considering the last term as the Bayes risk under squared loss, we can view the first term $\bbE\left[ \big( h\circ f(X) - \bbE[ Y \mid f(X) ] \big)^2 \right]$ as the excess risk.
%
% In Appendix \ref{sec:risk_decomp_additional}, we present a proof of Proposition \ref{Prop:risk_decomposition}, along with more detailed discussions on MSE decomposition and a unified geometric viewpoint on the relationship between various `recalibration scores' used in the literature.




\subsection{Problem Formulation: Recalibration}  \label{sec:setup}
Proposition \ref{Prop:risk_decomposition} motivates us to define the \emph{recalibration risk} of $g$ given $f$ as follows:
\begin{equation}\label{eqn:risk_recalib}
    R_P(h; f) := \bbE_P \left[(h\circ f(X) - \bbE_P[Y \mid f(X)])^2 \right].
\end{equation}
We may suppress the dependency on $f$ and $P$ and write $R(h) = R_P(h; f)$ to focus on its behavior with respect to $h$.
Note that $R(h) = 0$ if and only if $\REL(h \circ f; P) = 0$ and $\GRP( h; f, P) = 0$. 
This happens if and only if $h \circ f$ is calibrated, and $h \circ f (X)$ is sufficient for $f(X)$ with respect to $Y$. 
If $R(h) = 0$, then we call $h$ an \emph{optimal recalibration} of $f$ under $P$. 
Let $\hopt: \cZ \to \cZ$ be the function such that
\begin{equation}\label{eqn:optimal_h}
    \hopt(z) = 
        \begin{cases}
            \bbE_P [Y \mid f(X)=z],    &   \text{if }  z \in \supp P_{f(X)},\\
            0,                      &   \text{if }  z \not\in \supp P_{f(X)}.
        \end{cases}
\end{equation}
% \zs{Is $h^*$ undefined at $z_0=0.8$ if $\textrm{supp}(P_{f(X)}) = [0, 0.6]$? If function values on a null set don't matter, can we just set it as 0 for clarity?}
Then $R(\hopt) = 0$. Indeed, $h$ is an optimal recalibration of $f$ if and only if $h = \hopt$ $P_Z$-almost surely.

\begin{problem}[Recalibration]\label{problem:recalibration}
    Suppose that we have a measurable function $f: \cX \to \cZ$ and a dataset $\cD = \big\{ (x_i, y_i): i \in [n] \big\}$ that is an independent and identically distributed (IID) sample drawn from $P$. 
    The goal of \emph{recalibration} is to estimate $\hat{h} \approx \hopt$ using $f$ and $\cD$. 
\end{problem}

\begin{remark}
    We note that the aim of recalibration (Problem \ref{problem:recalibration}) is not in estimating $\bbP\left[ Y = 1 \mid X \right]$, which cannot be achieved unless $\sigma\big( f(X) \big) = \sigma(X)$. 
    Rather, its objective is post-process a pre-trained model $f$ to make them better calibrated, while preserving its sharpness. 
\end{remark}

% A common approach to tackle Problem \ref{problem:recalibration} is by minimizing the empirical risk $\hat{R}$ over a pre-defined hypothesis class $\cH$:
% \begin{equation}
%     \hat{h} = \argmin_{h\in\mathcal{H}} \hat{R}(h)
% \end{equation}
% The following are examples of the hypothesis class $\cH$ for some popular recalibration methods.


% \begin{example}[Platt scaling; \cite{platt1999probabilistic}]
%     Platt scaling uses the risk for the logistic loss and considers a parametric family of hypotheses $\mathcal{H}^{\mathrm{Platt}} = \left\{h(z)=\sigma(a z + b): a, b \in \mathbb{R} \right\}$, where $\sigma(z)=1/(1+e^{-z})$ is the sigmoid function. 
% \end{example}

% \begin{example}[Histogram binning; \cite{zadrozny2001obtaining}]
%     Histogram binning considers a family of monotone non-decreasing piecewise constant functions, $\mathcal{H}^{\mathrm{Hist}} = \left\{h(z)=\sum_{b=1}^B \mu_b \cdot \indic_{(u_{b-1}, u_b]}(z): B \in \NN \text{ and } u_0 \leq \dots \leq u_B \right\}$.
% \end{example}

% \DS{TODO: add a segway to the uniform-mass histogram binning described in the next section; it is not explicitly minimizing the empirical risk}







% \begin{example}[Uniform-mass binning]
% Uniform-mass binning \citep{zadrozny2001obtaining} uses $\mathcal{H}^{\textrm{UM}}_B(\{z_i\}_{i=1}^n) = \{h(z)=\sum_{b=1}^B \mu_b 1_{I_b}(z): I_b = (z_{(n(b-1)/B)}, z_{(nb/B)}], \mu_b\in [0, 1], \forall b \in [B]\}$
% \end{example}

% \begin{example}[Isotonic regression]
% Isotonic regression \citep{zadrozny2002transforming} uses $\mathcal{H}^{\textrm{ISO}} = \{h: h \textrm{ is monotonic}\}$. %$(z)=\sum_{b=1}^B \mu_b 1_{I_b}(z): \mu_b\in [0, 1], \mu_{b-1} < \mu_b, \forall b \in [B]\}$
% %$\mathcal{H}^{\textrm{Iso}}(\{z_i\}_{i=1}^n)
% \end{example}



==> archive/old_appx_not_used.tex <==
\section{Label Shift Correction Formula for $K \geq 2$}
\label{appendix:elkan}

We first derive the label shift correction formula under the general $K$-class classification, and then reduce to the binary classification.

In $K$-class classification problem with feature $X$ and target $Y$, the label shift assumption on distribution $P$ and $Q$ requires that:
\begin{align}
    \textrm{$P[X\in B | Y=k] = Q[X\in B | Y=k]$ for any $k \in \{1,2,\dots,K\}$ and any Borel set $B$.}
\end{align}
In addition, for regularity, we assume $Q_Y$'s support is covered by $P_Y$'s support; that is, $Q[Y=k] = 0$ whenever $P[Y=k] = 0$.

\begin{theorem}[Extension of \cite{elkan2001foundations} to $K$-classes]
Consider the $K$-class classification problem with feature $X$ and target $Y\in[K]$.
Let $\Delta_{\mathcal{Y}} = \{\alpha\in\RR^K: \sum_{k=1}^K \alpha_k = 1, \alpha_k \geq 0, \forall k\in[K]\}$.
Let $w = [w_1, \dots, w_K]$ with $w_k=Q[Y=k]/P[Y=k]$.
Define $g: \DY\to\DY$ as $g(\alpha) = [g_1(\alpha), g_2(\alpha), \dots, g_K(\alpha)]$, where
\begin{align}
    g_k(\alpha) = \frac{w_k \alpha_k}{\sum_{j=1}^K w_j \alpha_j}, \label{eq:g}
\end{align}
then we have
\begin{align}
    Q[Y=\cdot|X\in B] = g(P[Y=\cdot|X\in B]). \label{eq:posterior_adjust}
\end{align}    
\end{theorem}

\begin{proof}
For any class $k$ and any Borel set $B$ on $\calX$, we apply the Bayes rule on both $\bbP$ and $\bbQ$:
\begin{align}
    \bbP[Y=k|X\in B] &= \frac{\bbP[Y=k]}{\bbP[X\in B]} \bbP[X\in B|Y=k], \\
    \bbQ[Y=k|X\in B] &= \frac{\bbQ[Y=k]}{\bbQ[X\in B]} \bbQ[X\in B|Y=k].
\end{align}
Noticing the class conditional distribution are the same under the label shift assumption, we have
\begin{align}
    \bbQ[Y=k|X\in B] &= \frac{\bbQ[Y=k]}{\bbP[Y=k]}\frac{\bbP[X\in B]}{\bbQ[X\in B]} \bbP[Y=k|X\in B]. \label{eq:ls_1}
\end{align}
Summing over $k$ yields
\begin{align}
    1 &= \sum_{j=1}^K \frac{\bbQ[Y=j]}{\bbP[Y=j]}\frac{\bbP[X\in B]}{\bbQ[X\in B]} \bbP[Y=j|X\in B]. \label{eq:ls_2}
\end{align}
Dividing Equation~(\ref{eq:ls_1}) by Equation~(\ref{eq:ls_2}), we have
\begin{align}
    \bbQ[Y=k|X\in B] &= \frac{\frac{\bbQ[Y=k]}{\bbP[Y=k]}\frac{\bbP[X\in B]}{\bbQ[X\in B]} \bbP[Y=k|X\in B]}{\sum_{j=1}^K \frac{\bbQ[Y=j]}{\bbP[Y=j]}\frac{\bbP[X\in B]}{\bbQ[X\in B]} \bbP[Y=j|X\in B]} \\
    &= \frac{\frac{\bbQ[Y=k]}{\bbP[Y=k]} \bbP[Y=k|X\in B]}{\sum_{j=1}^K \frac{\bbQ[Y=j]}{\bbP[Y=j]} \bbP[Y=j|X\in B]} \\
    &= \frac{w_k \bbP[Y=k|X\in B]}{\sum_{j=1}^K w_j \bbP[Y=j|X\in B]} \label{eq:ls_0} \\
    &= \bbQ[Y=\cdot|X\in B] = g(\bbP[Y=\cdot|X\in B]). %\label{eq:posterior_adjust}
\end{align}
% where we have denoted $\bbQ[Y=k] / \bbP[Y=k]$ as $w_k$, referred to as the \emph{importance weight} for class $k$\footnote{The name "importance weight" comes from importance sampling, where we need to reweight the integrand when taking expectation under a different measure. More formally, the importance weight is the Radon-Nicodym derivative between the two distributions $W=\frac{dQ}{dP}$. By the definition of Radon-Nicodym derivative, $E_Q[Z] = E_P[WZ]$. Represented as densities, the importance weights are $w(x,y)=\frac{q(x,y)}{p(x,y)}$. Under label shift, the importance weight reduces to the class proportion ratios $w(x,y)=\frac{q(y)}{p(y)}$}.

% Define the \emph{label-shift recalibration} function $g: \DY\to\DY$ as $g(\alpha) = [g_1(\alpha), g_2(\alpha), \dots, g_K(\alpha)]$, where
% \begin{align}
%     g_k(\alpha) = \frac{w_k \alpha_k}{\sum_{j=1}^K w_j \alpha_j}, %\label{eq:g}
% \end{align}
% then Equation~\ref{eq:ls_0} can be rewritten as
% \begin{align}
%     \bbQ[Y=\cdot|X\in B] = g(\bbP[Y=\cdot|X\in B]). %\label{eq:posterior_adjust}
% \end{align}    
\end{proof}

% \todo{prove the binary case}
In binary classification, $k$ takes value 0 or 1, and we take the component of $g_1$ correspond to $k=1$, and denote it as $g_w$ in the rest of the paper:
\begin{align}
    g_w(\alpha) = \frac{w_1 \alpha}{w_1 \alpha + w_0 (1 - \alpha)},\quad \alpha\in[0,1]. \label{eq:g_bin}
\end{align}





\subsection{Lemmas that are no longer used}


\begin{lemma}\label{LEMMA:OPQ}
Suppose $P$ and $Q$ satisfy Assumption~\ref{assumption:label_shift} and \ref{assumption:in_training}. Let $\{X_n: n\in[N]\}$ and $\{R_n: n\in[N]\}$ be two sequences of random variables. Then $X_n = O_P(R_n)$ if and only if $X_n = O_Q(R_n)$. In other words, $O_P(R_n) = O_Q(R_n)$.
\end{lemma}
\begin{proof}
    Suppose $X_n = O_P(R_n)$, then $\sup_n P[|X_n / R_n| > K] \to 0$ as $K \to 0$. Then, by Lemma~\ref{LEMMA:W},
    \begin{align}
        \sup_n Q[|X_n / R_n| > K] \leq M \sup_n P[|X_n / R_n| > K] \to 0, \textrm{ as $K \to \infty$.}
    \end{align}
    So $X_n = O_Q(R_n)$. The other direction follows by symmetry.
\end{proof}



\begin{lemma}[\zs{Not used}]
Suppose $P$ and $Q$ satisfy the Assumption~\ref{assumption:label_shift} and \ref{assumption:in_training}. For any event $A$ and $B$ such that $P[A] < \epsilon_1$ and $Q[B] < \epsilon_2$ for some $\epsilon_1, \epsilon_2\in (0,1)$, we have
$$Q[A \cup B] < M \epsilon_1 + \epsilon_2,$$
where $M = \max_{k\in[K]} Q[Y=k]/P[Y=k]$
\end{lemma}
\begin{proof}
Define $w:[K]\to\RR$ as $w(k)=Q[Y=k]/P[Y=k]$, then $M=\max_{k\in[K]} w(k)$.
\begin{align}
    Q[A\cup B] &\leq Q[A] + Q[B] \comment{Union bound} \\
    &= E_P[w(Y) P[A|Y]] + Q[B] \comment{Lemma~\ref{LEMMA:W}} \\
    &\leq E_P[M P[A|Y]] + Q[B] \\
    &= M P[A] + Q[B] \\
    &\leq M \epsilon_1 + \epsilon_2.
\end{align}
\end{proof}


We need another lemma before proving Theorem~\ref{THM:MAIN}.

\begin{lemma}\label{LEMMA:BER}
    Suppose $\{Y_i: i\in[N]\}$ are i.i.d Bernoulli$(\pi)$, where $\pi = P[Y=1]$. The sample mean $\hat{\pi}=\frac{1}{N}\sum_{i=1}^N Y_i$ estimates $\pi$ with error $\hat{e} = \pi - \hat{\pi}$. For any $\epsilon > 0$,
\end{lemma}
\begin{proof}
The random variables $Y_i$ are bounded by [0,1]. By Hoeffding's inequality\footnote{This lemma can also been shown using Chebyshev's inequality. The factor $1/\sqrt{N}$ in the error is the same, the difference is the $\delta$ factor.}, for any $\epsilon > 0$,
\begin{align}
    P\left[ \left| \hat{\pi} - \pi \right| > \epsilon \right] \leq 2 e^{-2n\epsilon^2}.
\end{align}
Then the error $\hat{e} = \pi - \hat{\pi} = O_P(N^{-1/2})$ since $\sup_n P\left[ \left| \frac{\hat{e}}{1/\sqrt{n}} \right| > K \right] = \sup_n P\left[ |\hat{e}| > \frac{K}{\sqrt{n}}\right] \leq 2e^{-2K} \to 0$ as $K\to \infty$. 
\end{proof}




% 4 properties of autocalibration
% \section{Proof of Proposition~\ref{PROP:AUTO}}
% \label{appendix:auto}
% \begin{proof}
% \begin{enumerate}
%     \item For any $Z\in\mathcal{S}$,
%     \begin{align}
%         \eta(\eta(Z)) &= E[Y|\eta(Z)] \\
%         &= E[E[Y|Z]|\eta(Z)] \\
%         &= E[E[Y|\eta(Z) | Z] \\
%         &= E[Y|\eta(Z)] \\
%         &= \eta(Z).
%     \end{align}
%     \item 
%     \begin{align}
%         \eta(Z_c) = \eta(EY) = E[Y|EY] = EY = Z_c
%     \end{align}
%     \item This is just saying $\mathcal{S}$
% \end{enumerate}
% \end{proof}

\section{Zeyu's Attempt for the Proof of Theorem~\ref{THM:MAIN}}



\subsection{Useful Lemmas}
This section presents some useful results of label shift assumption. We first introduce the importance weights, which play an importance role in the results.

\marginnote{importance weights}
The label shift is fully characterized by the function $w:[K]\to\RR$ defined as
\begin{align}
    w(k) = \frac{Q[Y=k]}{P[Y=k]}. \label{eq:w}
\end{align}
% It can be also viewed as a vector $\underline{w}\in\RR^K$, which is often referred to as the importance weights\footnote{The name "importance weight" comes from importance sampling, where we need to reweight the integrand when taking expectation under a different measure. More formally, the importance weight is the Radon-Nicodym derivative between the two distributions $W=\frac{dQ}{dP}$. By the definition of Radon-Nicodym derivative, $E_Q[Z] = E_P[WZ]$. Represented as densities, the importance weights are $w(x,y)=\frac{q(x,y)}{p(x,y)}$. Under label shift, the importance weight reduces to the class proportion ratios $w(x,y)=\frac{q(y)}{p(y)}$} \cite{lipton2018detecting}.
We refer to the random variable $W=w(Y)$ as the importance weight variable\footnote{In general, the importance weight variable is the Radon-Nikodym derivative of $Q$ w.r.t. $P$: $W=\frac{dQ}{dP}$. Under the label shift assumption, this reduces to $W = \frac{dQ_Y}{dP_Y}$.}.
% When change the distribution of expectation, we need to multiply a random variable.


\begin{lemma}
\label{LEMMA:W}
Suppose $P$ and $Q$ satisfy the Assumption~\ref{assumption:label_shift} and \ref{assumption:in_training}, and let $w:[K]\to\RR$ be defined in Equation~(\ref{eq:w}). Then, for any measurable function $f:\mathcal{X}\to\RR$, we have:
\begin{enumerate}[label=(\alph*)]
    \item $E_Q[f(X)] = E_P[w(Y) E_P[f(X)|Y]].$
    \item $E_Q[f(X)] \in [m E_P[f(X)], M E_P[f(X)]], \textrm{ where } m=\min_{k\in[K]} w(k)$ and $M=\max_{k\in[K]} w(k).$
\end{enumerate}
\end{lemma}

\begin{proof}
\begin{align}
    E_Q[f(X)] &= E_Q[E_Q[f(X) | Y]] \\
    &= \sum_{k=1}^K Q[Y=k] E_Q[f(X) | Y] \\
    &= \sum_{k=1}^K P[Y=k] w(k) E_Q[f(X) | Y] \\
    &= \sum_{k=1}^K P[Y=k] w(k) E_P[f(X) | Y] \\
    &= E_P[ w(Y) E_P[f(X) | Y]].
\end{align}
Since $m\leq w(Y) \leq M$ and $E_P[f(X) | Y] \geq 0$, we can bound $E_Q[f(X)]$:
\begin{align}
    E_Q[f(X)] \in [m E_P[f(X)], M E_P[f(X)]].
\end{align}
\end{proof}


\begin{lemma}[Properties of $g_w$]\label{LEMMA:LIP}
    $g_w(z)$ is Lipschitz with constant $\frac{M}{m}$, where $M=\max\{w_0, w_1\}$ and $m=\min\{w_0, w_1\}$.
\end{lemma}
\begin{proof} We have
\begin{align}
    g_w(z) &= \frac{w_1 z}{w_1 z + w_0 (1-z)} \\
    g'_w(z) &= \frac{w_1 w_0}{(w_1 z + w_0 (1-z))^2}
    \leq \max\{ g'_w(0), g'_w(1) \}
    = \max\left\{ \frac{w_1}{w_0}, \frac{w_0}{w_1} \right\}
    = \frac{M}{m}.
\end{align}
Therefore, $g'_w(z) \in (0, M/m]$.

For any $z_1 < z_2 \in [0, 1]$, by Mean Value Theorem, there is $\tilde{z}\in [z_1, z_2]$ such that
\begin{align}
    g_w(z_1) - g_w(z_2) &= g_w(\tilde{z}) (z_1 - z_2).
\end{align}
Therefore, we have
\begin{align}
    | g_w(z_1) - g_w(z_2) | &= | g_w(\tilde{z}) (z_1 - z_2) | \\
    &\leq \max_z |g_w(z)| |z_1 - z_2| \\
    &= \frac{M}{m} |z_1 - z_2|.
\end{align}
\end{proof}



\subsection{Completing the Proof of Theorem~\ref{THM:MAIN}}
\label{appendix:main_theorem}


Recall Theorem~\ref{THM:MAIN}:
\main*
% \newcommand{\RQ}{R_{\mathbb{Q}}}
% \newcommand{\hhQ}{\hat{h}_{\mathbb{Q}}}
% \newcommand{\hhP}{\hat{h}_{\mathbb{P}}}
% \newcommand{\gh}{g_{\hat{w}}}

\begin{proof}
\begin{align}
R_Q\left(\hat{h}_Q\right)
&=E_Q\left[\left(\hat{h}_Q(Z)-E_Q\left[Y \mid \hat{h}_Q(Z)\right]\right)^2\right] \\
&=E_Q\left[\left(\hat{h}_Q(Z)-E_Q\left[E_Q\left[Y \mid \hat{h}_P(Z)\right] \mid \hat{h}_Q(Z)\right]\right)^2\right] \quad\quad (\textrm{Since }\hat{h}_Q(Z) = g_{\hat{w}}(\hat{h}_P(Z))) \\
& \leq E_Q\left[E_Q\left[\left(\hat{h}_Q(Z)-E_Q\left[Y \mid \hat{h}_P(Z)\right]\right)^2 \mid \hat{h}_Q(Z)\right]\right] \quad\quad (\textrm{Jensen's inequality}) \\
& =E_Q\left[\left(\hat{h}_Q(Z)-E_Q\left[Y \mid \hat{h}_P(Z)\right]\right)^2\right] \\
& \leq E_Q\left[\left|\hat{h}_Q(Z)-E_Q\left[Y \mid \hat{h}_P(Z)\right]\right|\right] \\
& =E_Q\left[\left|g_{\hat{w}}\left(\hat{h}_P(Z)\right)-g_w\left(E_P\left[Y \mid \hat{h}_P(Z)\right]\right)\right|\right] \\
& \leq E_Q\left[\underbrace{\left|g_{\hat{w}}\left(\hat{h}_P(Z)\right)-g_w\left(\hat{h}_P(Z)\right)\right|}_{T_1}\right] + E_Q\left[\underbrace{\left|g_w\left(\hat{h}_P(Z)\right)-g_w\left(E_p\left[Y \mid \hat{h}_P(Z)\right]\right)\right|}_{T_2}\right] \label{eq:comb} \end{align}

To bound $E_Q T_2$, we use the same derivation in Equation
\begin{align}
E_Q T_2 & \leq \frac{M}{m} E_Q \left|\hat{h}_P(Z)-E_P\left[Y \mid \hat{h}_P(Z)\right]\right| \comment{Lemma~\ref{LEMMA:LIP}} \\
& \leq \frac{M^2}{m} E_P\left|\hat{h}_P(Z)-E_P\left[ Y \mid \hat{h}_P(Z)\right]\right| \comment{Lemma~\ref{LEMMA:W}} \\
& \leq \frac{M^2}{m} \sqrt{\frac{4}{c B}} \quad\quad 
\begin{aligned}
    &\textrm{w.p.} \geq 1-\delta, \forall \delta\in(0,1), \\
    &\textrm{ if } n \geq c B^2 \log (B / \delta),  B \geq 4 \delta
\end{aligned}
&& (\textrm{by Equation (\ref{eq:60})-(\ref{eq:66})}) \label{eq:T2} \\
\end{align}

To bound $T_1$, we first define some shorthand notations. Let $\pi = P[Y=1]$, $\pi'=Q[Y=1]$. Then $w_1 = \pi'/\pi$ and $w_0 = (1-\pi') / (1-\pi)$. Define odds-ratio
\begin{align}
    r &= \frac{w_0}{w_1} = \frac{((1-\pi')\pi'}{(1-\pi)\pi'} \\
    &= \underbrace{\left(\frac{1}{\pi'} - 1\right)}_{:=a} \underbrace{\left(\frac{1}{\pi} - 1\right)^{-1}}_{:=b} \\
    &= ab.
\end{align}

\paragraph{Bounding the estimation errors for $\pi$ and $\pi'$}
\newcommand{\eps}{\epsilon_{\delta}}
Denote the sample mean for the labels on the training set and the test set as, respectively,
\begin{align}
    \hat{\pi} = \frac{1}{N}\sum_{i=1}^N y_i, \quad \hat{\pi}' = \frac{1}{N'}\sum_{i=1}^{N'} y'_i.
\end{align}
Let $\hat{e}=\hat{\pi}-\pi$ and $e^{\prime}=\hat{\pi}^{\prime}-\pi^{\prime}$. By Hoeffding's inequality, for any $\delta \in(0,1)$,
\begin{align}
P[|\hat{e}|>\epsilon_{\delta}] \leq \delta, \quad \textrm{and} \quad
Q\left[\left|\hat{e}^{\prime}\right|>\epsilon'_{\delta}\right] \leq \delta,
\end{align}
where
\begin{align}
\eps = \sqrt{\frac{1}{2 N} \log \frac{2}{\delta}}, \quad \textrm{and} \quad
\eps' = \sqrt{\frac{1}{2 N^{\prime}} \log \frac{2}{\delta}}=\sqrt{\frac{N}{N^{\prime}}} \eps := \lambda \eps .
\end{align}
Then
\begin{align}
& Q\left[|\hat{e}|>\eps \text { or }\left|\hat{e}^{\prime}\right|>\eps'\right] \\
\leq & Q[|\hat{e}|>\eps]+Q\left[\left|\hat{e}^{\prime}\right|>\eps'\right] &\textrm{(union bound)} \\
\leq & M P[|\hat{e}|>\eps]+Q\left[\left|\hat{e}^{\prime}\right|>\eps'\right] &\textrm{(Lemma~\ref{LEMMA:W}(b))} \\
\leq & (M+1) \delta.
\end{align}
So the event
\begin{align}
    E: \quad |\hat{e}| \leq \eps \text { and }\left|\hat{e}^{\prime}\right| \leq \eps'
\end{align}
occurs with probability at least $1 - (M+1)\delta$ under distribution $Q$.

\paragraph{Bounding the estimation errors for $a$ and $b$}
\newcommand{\ea}{\hat{e}_a}
\newcommand{\eb}{\hat{e}_b}
Let
\begin{align}
    \hat{a} = \frac{1}{\hat{\pi'}} - 1, \quad \textrm{and} \quad 
    \hat{b} = \left(\frac{1}{\hat{\pi}} - 1\right)^{-1}
\end{align}
and
\begin{align}
    \ea &= \hat{a} - a = \frac{-\hat{e}'}{\pi' (\pi' + \hat{e}')}, \\
    \eb &= \hat{b} - b
    = \frac{\frac{1}{\pi} - \frac{1}{\pi+\hat{e}}}{\left(\frac{1}{\pi+\hat{e}} - 1\right) \left(\frac{1}{\pi} - 1\right)}
    = \frac{\hat{e}}{(1 - \pi - \hat{e})(1 - \pi)}.
\end{align}
By Assumption~\ref{assumption:label_shift} (B2) and (B3), there exists $\zeta > 0$ such that $\pi,\pi'\in[\zeta, 1-\zeta]$.
For large enough $N$ and $N'$, we have
\begin{align}
\eps \leq (\zeta / 2) \min \left\{1 , \lambda \right\}, \label{eq:solve_n_from_ab}
\end{align}
then $\eps \leq \zeta/2$ and $\eps' \leq \zeta/2$. Thus $\pi' - \eps' \geq \pi' / 2$ and $1 - \pi - \eps \geq (1 - \pi) / 2$.
Therefore, under the event $E$,
\begin{align}
    |\ea| &\leq \frac{\eps}{\pi'(\pi' - \eps')} \leq \frac{2\eps'}{\pi'^2} = \frac{2\lambda\eps}{\pi'^2}, \\
    |\eb| &\leq \frac{\eps}{(1 - \pi - \eps)(1 - \pi)} \leq \frac{2\eps}{(1-\pi)^2}.
\end{align}

\paragraph{Bounding the estimation errors for $r$}
We have
\begin{align}
    \hat{r} &= \hat{a}\hat{b} \\
    &= ab + \ea b + \eb a + \ea \eb.
\end{align}
Then
\begin{align}
    \hat{e}_r
    &=|\hat{r} - r| \\
    &\leq |\ea| b + |\eb| a + |\ea| |\eb| \\
    &\leq \frac{2\lambda\eps}{\pi'^2} \frac{\pi}{1 - \pi} + \frac{2\eps}{(1-\pi)^2} \frac{1 - \pi'}{\pi'} + \frac{4\lambda\eps^2}{\pi'^2 (1-\pi)^2} \\
    &\leq \frac{2}{\pi'^2 (1-\pi)^2} \left[ \left( \lambda\pi(1-\pi) + \pi'(1-\pi') \right) \eps + 2\lambda \eps^2 \right] \\
    &\leq \frac{1}{2\pi'^2 (1-\pi)^2} \left[ (1 + \lambda) \eps + 8 \lambda \eps^2 \right] \\
    &\leq \frac{1}{2\zeta^4} \left[ (1 + \lambda) \eps + 8 \lambda \eps^2 \right] := \epsilon_r
\end{align}

\paragraph{Bounding the estimation errors for $g_w(\hat{h}_P(Z))$}
For brevity, let $\tilde{Z}=\hat{h}_P(Z)$.
\begin{align}
T_1
& =\left|g_{\hat{w}}(\tilde{Z})-g_w(\tilde{Z})\right| \\
& =\left|\frac{1}{1+\hat{r}(1 / \tilde{Z}-1)}-\frac{1}{1+r(1 / \tilde{Z}-1)}\right| \\
& =\frac{1 / \tilde{Z}-1}{(1+\hat{r}(1 / \tilde{Z}-1))(1+r(1 / \tilde{Z}-1))}|r-\hat{r}| \\
& \leq \frac{1 / \tilde{Z}-1}{\left(1+\frac{r}{2}(1 / \tilde{Z}-1)\right)(1+r(1 / \tilde{Z}-1))}|r-\hat{r}| &\text { if } \hat{r} \geq \frac{r}{2} \Leftarrow|\hat{e}_r| \leq \frac{r}{2} \Leftarrow|\epsilon_r| \leq \frac{m}{2 M} \\
& \leq \frac{1 / \tilde{Z}-1}{\left(1+\frac{r}{2}(1 / \tilde{Z}-1)\right)^2}|r-\hat{r}| \\
& \leq \frac{1}{r}|r-\hat{r}| \\
& \leq \frac{M}{m}|r-\hat{r}| &\textrm{$\left(r=\frac{w_0}{w_1} \geq \frac{m}{M}\right)$} \label{eq:solve_n_from_r} \\
& \leq \frac{M}{2m\zeta^4} \left[ (1 + \lambda) \eps + 8 \lambda \eps^2 \right]
\end{align}
So
\begin{align}
    E_Q T_1 \leq \frac{M}{2m\zeta^4} \left[ (1 + \lambda) \eps + 8 \lambda \eps^2 \right] \label{eq:T1}
\end{align}

Combining Equation~(\ref{eq:comb}), (\ref{eq:T2}) and (\ref{eq:T1}), we have the desired result:
with probability at least $1-(M+1)\delta$,
\begin{align}
R_Q\left(\hat{h}_Q\right)
&\leq \frac{M^2}{m} \sqrt{\frac{4}{c B}}
+ \frac{M}{2m\zeta^4} \left[ (1 + \lambda) \epsilon + 8 \lambda \epsilon^2 \right] \\
&\leq \frac{2 M^2}{m} \sqrt{\frac{1}{c B}}
+ \frac{M(1+\lambda)}{2\sqrt{2} m\zeta^4 \sqrt{N}} \log \frac{2}{\delta}
+ \frac{4M\lambda}{m\zeta^4 \sqrt{NN'}} \log \frac{2}{\delta},
\end{align}
if the sample sizes $N, N'$ satisfy the following conditions required by Equation~(\ref{eq:solve_n_from_ab}) and (\ref{eq:solve_n_from_r}):
\begin{align}
    \eps &\leq \frac{\zeta}{2} \min \{1, \lambda\}, \\
    \epsilon_r &\leq \frac{m}{2M}.
\end{align}
\end{proof}

\begin{remark}
Solving Equation~\ref{eq:solve_n_from_ab} yields the sample size requirement:
\begin{align}
    N, N' \geq \frac{2}{\zeta^2} \log \frac{2}{\delta}. \label{eq:n_require}
\end{align}

Solving Equation~\ref{eq:solve_n_from_r} yields the sample size requirement\todo{Find sufficient requirement for sample sizes}:
\begin{align}
    &\frac{1}{2\zeta^4} \left[ (1 + \lambda) \epsilon_{\delta} + 8 \lambda \epsilon_{\delta}^2 \right] \leq \frac{m}{2M} \\
    \Leftarrow\ &\frac{1}{2\zeta^4} \left[ (1 + \lambda) \epsilon_{\delta} + 8 \lambda \epsilon_{\delta} \right] \leq \frac{m}{2M} \\
    \Leftarrow\ &\frac{1}{2\zeta^4} \left[ (1 + 9 \lambda) \epsilon_{\delta} \right] \leq \frac{m}{2M} \\
    \Leftarrow\ &\epsilon_{\delta} \leq \frac{m\zeta^4}{M(1 + 9 \lambda)}
\end{align}
\end{remark}

% To bound $T_1$, we rewrite the label shift adjustment as
% \begin{align}
%     g_w(z) &= \frac{w_1 z}{w_1 z + w_0 (1-z)} \\
%     &= \frac{1}{1 + (w_0 / w_1) (1/z - 1)} \\
%     &= \frac{1}{1 + r (1/z - 1)}.
% \end{align}

% Abusing notations, define
% \begin{align}
%     g(r,z) = 1 / (1 + r (1/z - 1)).
% \end{align}

% \begin{align}
%     g(\hat{r}, z) - g(r, z) &= \frac{\partial}{\partial r} g(\Tilde{r}, z)(\hat{r} - r) \comment{for some $\tilde{r}$ in between $\hat{r}$ and r} \\
%     |g(\hat{r}, z) - g(r, z)| &\leq G \epsilon_r(\alpha) \quad\textrm{w.p. at least }1 - \alpha
% \end{align}

% $\tilde{r}\overset{p}{\to}r$, $\frac{\partial g}{\partial r}$ continuous at $r$, so the partial derivative also converges to the finite number in probability, say $G$. % What is this?

% \section{Concentration Inequalities}
% \label{appendix:concentration}

% \footnote{The materials in this section come from \url{https://www.stats.ox.ac.uk/~rebeschi/teaching/AFoL/20/material/lecture07.pdf}}

% \begin{definition}[One-sided Bernstein's condition]
% A random variable $X$ satisfies \emph{one-sided Bernstein's condition} with parameter $b > 0$ if
% $$
% E e^{\lambda(X-E X)} \leq \exp \left(\frac{(\var X) \lambda^2 / 2}{1-b \lambda}\right) \quad \text { for any } \lambda \in[0,1 / b).
% $$
% \end{definition}

% \begin{proposition}[Bernstein's upper-tail bound]
% Let $X$ be a random variable that satisfies the onesided Bernstein's condition with parameter $b>0$. Then, for any $\varepsilon \geq 0$, we have
% $$
% P[X-E X \geq \varepsilon] \leq \exp \left(-\frac{\operatorname{Var} X}{b^2} h\left(\frac{b \varepsilon}{\operatorname{Var} X}\right)\right) \leq \exp \left(-\frac{\varepsilon^2 / 2}{\operatorname{Var} X+b \varepsilon}\right).
% $$
% Or equivalently, for any $\delta \in(0,1)$,
% $$
% P[X-EX < b \log (1 / \delta)+\sqrt{2(\operatorname{Var} X) \log (1 / \delta)}] \geq 1-\delta
% $$
% \end{proposition}



==> archive/old_introduction.tex <==
\section{Introduction}

% In many classification problems, obtaining a predictor that accurately captures the distributional features of the data is crucial, especially for high-stakes applications where decision-makers require reliable information to make informed choices. 
% The ability to estimate functionals of the predictive distribution, such as confidence intervals, prediction sets, quantiles, or the distribution itself, is of great interest in these scenarios. 
% However, the performance of many machine learning models deteriorates when there is a distribution shift between the training and testing data.

% To address this issue, post-hoc probability recalibration methods have been proposed to adjust the model's predicted probabilities to match the true probabilities of the testing data. 
% However, many of these methods ignore the problem of decreased resolution of the post-hoc calibration or rely on heuristic or empirical methods that lack rigorous finite sample guarantees. 
% In this work, we study the problem of calibrating probabilistic classifiers while preserving their resolution as much as possible, which we refer to as \emph{sufficient probability calibration}.
% Our proposed approach is motivated by recent advances in statistical learning under distribution shift, which aim to obtain predictors that not only perform well in point-wise manner but also accurately capture the distributional features. 

% We develop a novel method for  sufficient probability calibration that leverages these advances, and demonstrate its effectiveness with both theoretical analysis and numerical experiments. 

% ====

\marginnote{motivate Sec~3: optimal calibration}
\zs{why probabilistic estimate}\zs{delete this or merge it into the second paragraph}
{\color{lightgray}
In many classification problems, obtaining a predictor that accurately captures distributional features of the data is crucial, especially for high-stakes applications such as medical diagnosis and space weather forecast.
In these applications, decision-makers require information on the predictive distribution to make informed choices.
The ability to estimate functionals of the predictive distribution, such as confidence intervals, prediction sets, quantiles, or the distribution itself, is of great interest in these scenarios.
}

\zs{why probabilistic calibration}
One particularly desirable attribute for probabilistic classifiers is \emph{reliability}, which refers to the consistency between the distribution estimate and the true conditional distribution given the observation.
However, many machine learning algorithms only give point classification, scores that can't be interpreted as probability, or probability estimates that are not reliable/calibrated due to various reasons (e.g., model misspecification).
To address this issue, post-hoc recalibration methods have been proposed to adjust the model's predicted probabilities \cite{zadrozny2001obtaining,zadrozny2002transforming,guo2017calibration,vaicenavicius2019evaluating,kumar2019verified}.
However, many of these methods ignore the problem of decreased resolution of the post-hoc calibration or rely on heuristic or empirical methods to preserve the prediction resolution that lack rigorous finite sample guarantees \citep{vaicenavicius2019evaluating,gupta2020predictionset,gupta2021withoutsplitting}.

\zs{what is our contribution in Sec~3 (optimal calibration)}
In this work, we formally establish a geometrically interpretable framework of constructing, analyzing, and diagonosing post-hoc recalibration methods that reaches the optimal finite sample error rate. We refer to the recalibration methods constructed using our framework as \emph{optimal probability calibration}, which enjoys the property of calibrating probabilistic classifiers while preserving their resolution as much as possible.
Our work is motivated by integrating a large literature on score decompositions in meteorology and machine learning community, dating back to brier score components in 50's and murphy's decomposition in 70's, to recent advances in machine learning and economics of proper scoring rule decomposition.

% Uncomment if we needs a brief intro to our method
% \marginnote{Why grouping risk is important}
% Popular nonparametric methods, such as histogram binning and isotonic regression using PAVA, all fits a piecewise constant function so there is grouping effect, which needs to be characterized to analyze the performance of recalibration. We propose to use a risk called grouping risk to evaluate the risk associated with the grouping. Note the risk has been proposed in the literature \zs{todo}.

\marginnote{motivate Sec~4: calibration under label shift}
\zs{why consider domain shift; popular adaptations \& limitations}
Domain shift is a prevalent problem in machine learning. It refers to the scenario when the task or data distribution on which we deploy our pretrained models are different than what the models are trained on, which can cause adaptation issues for the machine learning models. Many learning paradigms are proposed to address this issue.
Transfer learning requires fine-tuning on a sufficient amount of labeled target-domain data to avoid overfitting, since high dimensional features are involved. However, many times we do not have enough labeled data on the target domain due to the cost issues.
Few/Zero-shot learning requires specially-designed models/algorithms that are pre-trained on large datasets, which may not be true for the given classifier.
Meta learning requires specially-designed models/algorithms that are pre-trained on multiple tasks, which may not be true for the given classifier.

\zs{why consider label shift}
A specific type of domain shift is distribution shift.
A specific type of distribution shift is label shift, where the marginal probabilities of the classes on the training set is different from those on the test set.
Label shifts between domains are common. They can be intrinsic (e.g., flu and hay fever have similar symptoms, but prevalence depends on seasons or if there's a breakout of one of them) or induced (e.g., rebalancing the classes in the training set by subsampling the majority class to prevent learning a classifier that predicts the majority class all the time. To generalize to a new task with potential class imbalance, we need a small sample to estimate the new class priors.).
%% A previous version of motivation/intro to label shift
% The generalization of statistical learning methods hinges on the distribution similarity between the training data and the test data. However, in practice, it is common that the test set distribution is shifted from the distribution of the training data. One particular distribution shift is label shift, where the a priori probabilities of the classes on the training set is different from those on the test set. Assuming the class conditional are invariant under the label shift, one can adjust the predicted probability for each class under the label shift using the information of how much class proportions have shifted.

%% \zs{We don't even need to argue the value of combining them together if we decouple calibration and label shift}
%% \zs{defer this when we introduce baseline in experiments}
% \marginnote{application of sufficient probability calibration under label shift}
% However, if the probability predictions given by machine learning algorithms are not accurate even on the training distribution, there is no way that we can recover the true distribution on the test set using the label shift correction \zs{Baseline in the experiment}. Therefore, accurate and sufficient \zs{sufficient is not motivated} probabilistic predictions is a prerequisite for the label shift correction.

\zs{what is our setting in Sec~4 (calibration under label shift)}
In this paper, we consider a label shift setting where we have access to labeled samples from both the source and the target domain. Further, we assume the target domain sample is too small to construct a reliable classifier, but it is sufficient for estimating the label distribution.
This differs from the settings considered by recent literature on label shift, where the only data we have from the target domain is the unlabeled test data \cite{saerens2002adjusting,lipton2018detecting,azizzadenesheli2018regularized,alexandari2020maximum,garg2020unified}.
However, we argue that our setting is prevalent and practical:
\begin{enumerate}
    \item In many cases, we are allowed to collect some labeled data in the target domain to adapt a pre-trained model before deployment. This is common in online learning, where we repeatedly deploy models in the target domain and observe the labels/rewards as we go. \todo{citation}
    \item Nonetheless, labeling target domain data is often time-consuming, labor-intensive, or cost-ineffective. For example, collecting a moderately large sample of strong solar flares can take two solar cycles. For another example, for some rare diseases, it is more difficult to collect data from the positive samples than negative samples. 
    \item In many cases, the target-domain sample size is sufficient to estimate the marginal distribution of the classes (which can be characterized by a scalar in binary classification), but is too small to either fine-tune the classifier which involve distributions of the classes conditioned on high dimensional features, or recalibrate the classifier which involves fitting a potentially infinite dimensional function that transforms the predicted probabilities.
    % This is because estimating class priors q(y) is low-dimensional (in fact, just a scalar for the binary case), whereas fine-tuning the estimate of q(y|x) involves high-dimensional x, and recalibrate the estimate of q(y|z) requires fitting a potentially infinite-dimensional function from [0,1] to [0,1]. (q denotes density for the target distribution, and z = f(x) denotes the predicted probability)
\end{enumerate}

%\zs{what is our contribution in Sec~4}

\marginnote{summary}
\zs{what is contained in this paper}
We develop novel theoretical guarantees and interpretations to an existing calibration method called uniform-mass binning. We also develop theoretical guarantees under the presence of label shift. We demonstrate the tightness of our bound using both numerical simulations and a real world application in solar flare prediction.
% We consider the problem of deriving the optimal post-hoc modification to distribution predictions under label shift. Label shift assumes class proportions change between datasets with class conditionals held the same. The label shift can arise in two situations:
% \begin{itemize}
%     \item Intrinsic label shift, where the marginal distributions of the labels between the datasets are naturally different. For example, model trained on a dataset collected in the early stages of an epidemic needs to be adjusted on a more recent dataset collected at the peak of epidemic. If we assume the symptoms of an infectious disease don't change over the time, then this is an example of label shift. Another example is solar flare classification, where the training set and the test set are usually chosen from two periods in the different phases of a solar cycle with different event rate.
%     \item Induced label shift, which is an algorithmic artifact caused by class-wise resampling on one dataset. For example, in imbalanced classification, to improve the classification performance on the underrepresented classes, we first fit the algorithms to a rebalanced dataset where the sample sizes for different classes are equalized. The learned model has to be adjusted to work in the real world setting where classes are imbalanced.
% \end{itemize}


\subsection{Contributions}
Our contribution can be summarized as follows: \zs{One sentence for our own reference}
\begin{itemize}
    \item \zs{We bring the sufficiency to people's attention.} We define the problem sufficient probability calibration, which takes into account the loss of prediction resolution caused by the grouping effect of recalibration methods. Our risk decomposition exposes the contribution of both calibration and grouping to the risk function.
    \item \zs{We combine the convergence rates of the grouping risk \cite{kumar2019verified} and the reliability risk \cite{gupta2021withoutsplitting} and get the the finite-sample error bound for our risk function.} We derived the high-probability finite-sample error bounds for both the calibration loss and the grouping loss. We then utilize them to bound the risk of the uniform-mass binning recalibration method. This yields a final error bound of $O(1/\sqrt{B})$ when $n=\Omega(B^2\log B)$.
    \item \zs{Optimal number of bins for UMB} We provide an optimal number of bins for uniform-mass binning recalibration method: $B = 2 \left( \log \frac{1}{\delta} \right)^{-1/3} n^{1/3}$, where $n$ denotes the sample size for the calibration data and $\delta$ denotes the upper bound for the failure probability of the upper bounds. This choice of $B$ is verified by numerical experiments.
    \item \zs{Label shift procedure with finite-sample error guarantee}  We show the label shift procedure preserves the optimality of calibration function: if the calibration function has small exess risk on one distribution, the label shift procedure ensures the calibration after label shift also achieves small risks under label shift. We provide finite-sample error guarantee for the label-shift-corrected recalibration function.
\end{itemize}

\subsection{Related Work}

\paragraph{Brier score decomposition.}
\zs{The following works only consider the empirical estimation of the scores. If forecast is continuous, this involves binning.}
\zs{From intro of \cite{stephenson2008two}} The Brier score is the mean squared difference between issued forecast probabilities and observed binary outcomes \cite{brier1950verification}. The Brier score can be decomposed into three components: forecast reliability, forecast resolution, and observation uncertainty \cite{sanders1963subjective,murphy1973new}.
For the continuous forecasts, binning is commonly used to empirically evaluate the components. This induces error in reliability risk and grouping risk, and introduces two other terms in the Brier score decomposition, within-bin variance (WBV) and within-bin covariance (WBC) \citet{stephenson2008two}.
\citet{kull2014reliability} proposed 7 components in a proper scoring rule, one of which is grouping loss. We name grouping risk after their work.

In empirical estimation with finite sample, bias correction has been proposed \cite{brocker2012estimating,scholkopf2012causal,kumar2019verified,lee2022t}. Ferro: bias(REL) decays at rate 1/n2.

\paragraph{Proper scoring rules.}
Logarithm scores are proposed with a similar REL-RES-UNC decomposition \cite{weijs2010kullback}.

\paragraph{Recalibration methods.}
\marginnote{parametric \& nonparametric}
Post-hoc probability calibration methods in binary classification can be categorized into parametric methods and nonparametric methods.
Parametric methods for calibration such as Platt scaling \cite{platt1999probabilistic}, temperature scaling \cite{guo2017calibration}, Beta calibration \cite{kull2017beyond}, and Dirichlet calibration \cite{kull2019beyond} model $h$ in some parametric form and use calibration data to estimate parameters. It has been shown that methods like Platt scaling are less calibrated than reported and it is difficult to estimate the degree of miscalibration\cite{kumar2019verified}\footnote{``If f(X) is continuous, without smoothness assumptions on E[Y | f(X)] (that cannot be verified in practice), this is impossible. This is analogous to the difficulty of measuring the mutual information between two continuous signals."\cite{kumar2019verified}}.
Nonparametric methods such as histogram methods using equal-width binning \cite{guo2017calibration} and uniform-mass-binning \cite{zadrozny2001obtaining} are popular due to lack of parametric assumptions. Isotonic regression impose a monotonicity assumption on the calibration function \cite{zadrozny2002transforming}. Gaussian processes are also used in the literature \cite{wenger2020non}.
% which assumes smoothness of $h$, and isotonic regression which assumes the monotonicity of $h$.

\marginnote{binning schemes}
% \paragraph{Histogram binning schemes in recalibration methods.}
In histogram methods, there have been several recent works on deciding the binning scheme.
Perhaps the most direct scheme is uniform-length binning scheme, which divides the interval [0,1] into a prespecified number of segments of equal length.
\cite{zadrozny2001obtaining} used a data-dependent uniform-mass binning scheme, which uses the quantiles of the predicted probabilities to determine the bin boundaries.
\cite{zadrozny2002transforming} proposed to use isotonic regression in calibration, for which the bins are the by-products of the pooled-adjacent-violator algorithm \cite[PAVA;][]{ayer1955empirical}.
\cite{naeini2015obtaining} proposed a Bayesian binning method that treats the number of bins as a random variable with a uniform prior in some range.
\cite{kumar2019verified} requires the uniform-mass binning scheme as opposed to equal-width binning to estimate the calibration error. They claim that equal-width binning makes measuring the calibration error less efficient, but it can improves the bounds on the MSE if the binning scheme turns out to be 2-well-balanced. This motivates a hybrid binning scheme. They think analyzing what binning scheme lead to the best bounds and seeing whether it can improve the calibration method is a good direction for future research.
\cite{roelofs2022mitigating} found equal-mass binning have lower bias than equal-width binning. They also proposed a method that choose the number of bins to be as large as possible while preserving monotonicity in the calibration function.
\cite{gupta2021withoutsplitting} gave a proof of the calibration guarantee of the uniform-mass-binning.
\cite{sulewski2021equal} empirically compared methods of equal-bin-width histograms (EBWH) and equal-bin-count histograms (EBCH), and recommend EBWH for symmetric distributions and EBCH otherwise.

In controlling the grouping loss, recent literature typically make assumptions or ad-hoc decisions. \cite{gruber2022better} restrict recalibration functions to injective transformations to avoid reducing models' sharpness. \zs{We also have }. This precludes the histogram binning methods. Instead, we do not make such assumptions, 

\paragraph{Data-dependent binning scheme.}

Optimal number of bins. Scott same rate.

\paragraph{Distribution shift / Out-of-sample generalization.}
\DS{Please fill this in.}

\paragraph{Label shift with labeled test data}
Our task of recalibration under label shift is motivated by the labeled dataset assumes access to labeled data on both the source and target domains, but the target domain sample is too small to construct a reliable classifier. However, it is sufficient for estimating the label distribution.

\paragraph{Label shift with unlabeled test data}
\cite{saerens2002adjusting} introduced the \emph{confusion matrix approach} (CM) and the \emph{maximum likelihood approach} (ML). The developed the EM algorithm for ML. No consistency results were given.
\cite{lipton2018detecting} rediscovered the CM, and proved its consistency and gave a bound for sample complexity.
\cite{azizzadenesheli2018regularized} reformulated CM approach using regularized least square estimation and derived a bound for the estimated weight shift. Based on that, they derived a generalization bound for the classifier importance reweighted ERM.
\cite{alexandari2020maximum} proposed to calibrate the classifier before performing ML approach to adapt to label shift. They verified empirically that ML with calibrated classifier works better than CM. They proved the convergence of the EM algorithm, by discovering that the ML objective is in fact concave.
\cite{garg2020unified}, also in Lipton's group, proposed a framework to unify CM and ML. They claimed both CM and ML are matching the distribution in the latent space. They gave the consistency results and sample complexity bound for ML.

\paragraph{Importance of calibration in label shift correction}
\cite{esuli2020critical} empirically showed EM approach \cite{saerens2002adjusting} only when the number of classes in the classification scheme is very small and the classifier is calibrated.
\cite{alexandari2020maximum} also find the same empirical results.
\cite{garg2020unified} provide theoretical reasons for why calibration is important by identify the calibration error term in the estimation error of the importance weights.

\subsection{Organization}
